Opetopic algebras I: Algebraic structures on opetopic sets

We define a family of structures called "opetopic algebras", which are algebraic structures with an underlying opetopic set. Examples of such are categories, planar operads, and Loday's combinads over planar trees. Opetopic algebras can be defined in two ways, either as the algebras of a "free pasting diagram" parametric right adjoint monad, or as models of a small projective sketch over the category of opetopes. We define an opetopic nerve functor that fully embeds each category of opetopic algebras into the category of opetopic sets. In particular, we obtain fully faithful opetopic nerve functors for categories and for planar coloured Set-operads. This paper is the first in a series aimed at using opetopic spaces as models for higher algebraic structures.

==> macros.tex <==
%
% macros.tex
% v2.2 2019/02/15
%

\makeatletter

% ------------------------------------------------------------------------------
% AUTOMATA
% ------------------------------------------------------------------------------

\newcategory{\Auto}{}{A}{uto}

\newcommand{\acc}{\mathrm{acc}}
\newcommand{\init}{\mathrm{init}}
\DeclareMathOperator{\triv}{triv}

% ------------------------------------------------------------------------------
% CATEGORIES
% ------------------------------------------------------------------------------

\newcategory{\Ctx}{}{C}{tx} % Category of contexts (syntaxtic category)

% ------------------------------------------------------------------------------
% General
% ------------------------------------------------------------------------------

\DeclareMathOperator{\eqdef}{\coloneq}
\DeclareMathOperator{\equivdef}{:\!\equiv}
\DeclareMathOperator{\hash}{\#}
\newcommand{\condition}[1]{\textbf{\upshape{(#1)}}}

% ------------------------------------------------------------------------------
% OPETOPES
% ------------------------------------------------------------------------------

\newcategory{\PshO}{}{\widehat{\bbOO}}{}
\newcategory{\FinO}{}{F}{in\PshO}

\newcommand{\opetope}[1]{\left\lbrace\begin{matrix*}[l]#1\end{matrix*}\right.}
\newcommand{\degenopetope}[1]{\left\lbrace \!\! \opetope{#1} \right.}
\newcommand{\sep}{\leftarrow}

\newcommand{\optZero}{\filledlozenge}
\newcommand{\optOne}{\filledsquare}
\newcommand{\optInt}[1]{\mathbf{#1}}

\newcommand{\namedcoding}[1]{\left\lBrack #1 \right\rBrack^!}
\newcommand{\polycoding}[1]{\left\lBrack #1 \right\rBrack^{\mathrm{poly}}}
\newcommand{\unnamedcoding}[1]{{\left\lBrack #1 \right\rBrack^?}}

\newcommand{\optPolyFun}{\frakZZ}

\newcommand{\shape}[1]{#1^\natural}

\newcommand{\universal}{\filledtriangleright}

% ------------------------------------------------------------------------------
% POLYGRAPHS
% ------------------------------------------------------------------------------

\newcategory{\Pol}{}{P}{ol}
\newcommand{\MTO}{\triangledown}
\newcommand{\PolMTO}{\Pol^\MTO}

% ------------------------------------------------------------------------------
% POLYNOMIAL FUNCTORS
% ------------------------------------------------------------------------------

\newcategory{\PolyEnd}{}{P}{oly{\catEE}nd}
\newcategory{\PolyMnd}{}{P}{oly{\catMM}nd}
\newcategory{\Tree}{}{T}{ree}

\newcommand{\polynomialfunctor}[7]{
    \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,
        row sep = 2 em,
        column sep = 2 em,
        text height = 1.5ex,
        text depth = 0.25ex,
        ampersand replacement = \&] {
            \displaystyle{#1} \&
            \displaystyle{#2} \&
            \displaystyle{#3} \&
            \displaystyle{#4} \\
        };
        \path[->]
            (m-1-2) edge node [above] {$#5$} (m-1-1)
            (m-1-2) edge node [above] {$#6$} (m-1-3)
            (m-1-3) edge node [above] {$#7$} (m-1-4);
    \end{tikzpicture}
}

% ------------------------------------------------------------------------------
% PROOFTREES
% ------------------------------------------------------------------------------

\newenvironment{prooftree*}{\leavevmode\hbox\bgroup}{\DisplayProof\egroup}

% ------------------------------------------------------------------------------
% TIKZ
% ------------------------------------------------------------------------------

\newcommand{\DDownarrow}{
    \mathrel{
        \begin{tikz} [baseline=-3pt, rotate=-90]
            \draw [shorten >= 0pt, shorten <= 0pt]
                (0, 3pt)  -- ++(1.5ex, 0)
                (0, 1pt)  -- ++(1.5ex+1pt, 0)
                (0, -1pt) -- ++(1.5ex + 1pt, 0)
                (0, -3pt) -- ++(1.5ex, 0)
                (1.5ex - 1pt, 5pt)
                    to [in = 135, out = -75] (1.5ex + 2pt, 0)
                    to [out = -135, in = 75] (1.5ex - 1pt, -5pt);
		\end{tikz}
	}
}

% This command alows to import parts of tikz files. The ``main'' tag is imported
% by default, and other tags can be specified in 3rd argument as a comma
% separated list (with NO SPACES!). 2nd argument is file name, expected to be in
% ``tikz/'' subdir. 1st argument in is optional, and is the tikz scale factor
\usepackage{catchfilebetweentags}
\newcommand{\tikzinput}[3][1]{
	\begin{tikzpicture}
        \tikzset{scale = #1}
		\ExecuteMetaData[tikz/#2.tikz]{main}
		\@for\tmp:=#3\do{
			\ExecuteMetaData[tikz/#2.tikz]{\tmp}
		}
	\end{tikzpicture}
}


\newcommand{\pullbackcorner}{
    \ar[dr, phantom, "\lrcorner", very near start, shift right = 0ex]
}
\newcommand{\pushoutcorner}{
    \ar[dr, phantom, "\ulcorner", very near end, shift right = 0ex]
}

% ------------------------------------------------------------------------------
% TODO
% ------------------------------------------------------------------------------

%\newcommand{\TODO}[1]{\marginpar{\tiny #1}}

% ------------------------------------------------------------------------------
% TREES
% ------------------------------------------------------------------------------

\newcommand{\itree}[1]{\mathsf{I}_{#1}}
\newcommand{\ytree}[1]{\mathsf{Y}_{#1}}

\newcommand{\leafsymbol}{|}
\newcommand{\nodesymbol}{\bullet}

\DeclareMathOperator{\tree}{tr}
\DeclareMathOperator{\treewithleaf}{tr^{\leafsymbol}}
\DeclareMathOperator{\treewithnode}{tr^{\nodesymbol}}

\newcommand{\underlyingtree}[1]{\left\langle #1 \right\rangle}

\newcommand{\addr}{\&}

\newcommand{\subst}{\operatornamewithlimits{\smallsquare}}
\newcommand{\graft}{\operatornamewithlimits{\circ}}
\newcommand{\grafti}{\operatornamewithlimits{\tilde{\circ}}}
\DeclareMathOperator*{\biggraft}{\bigcircle}

\DeclareMathOperator{\src}{\mathsf{s}}
\DeclareMathOperator{\tgt}{\mathsf{t}}
\DeclareMathOperator{\edg}{\mathsf{e}}

\newcommand{\readdress}{\wp}
\newcommand{\substreaddress}{\chi}

\makeatother

==> tikz/common.tex <==
\usetikzlibrary{calc, decorations.pathmorphing, positioning}

% args: x, y, w, h, label, inner x, innner y
\newenvironment{TIKZZONE}[7]{
\begin{scope} [shift = {(#1, #2)}]
\draw [dotted] (0, 0) node [above right] {\small{\texttt{#5}}} -- (0, #4) -- (#3, #4) -- (#3, 0) -- cycle;
\begin{scope} [shift = {(#6, #7)}]
}{
\end{scope} \end{scope}
}

\tikzset{treeedge/.style = {above, sloped}}
\tikzset{treenode/.style = {circle, minimum size = 2pt, inner sep = 0, draw, fill}}

\newcommand{\blackwhitespoon}{-}
\newcommand{\DDownarrow}{|}
\newcommand{\optInt}[1]{\textbf{#1}}
\newcommand{\optOne}{\rightarrow}
\newcommand{\optZero}{\bullet}
\newcommand{\readdress}{P}
\newcommand{\RRightarrow}{-}
\newcommand{\Rrightarrow}{\equiv\!>}
\newcommand{\smalltriangleright}{>}
\newcommand{\src}{\mathsf{s}}
\newcommand{\system}{\textsc}
\newcommand{\tgt}{\mathsf{t}}
